Quantifying local heterogeneities in the 3D morphology of X-PVMPT battery electrodes based on FIB-SEM measurements

Organic electrode-active materials (OAMs) not only enable a variety of charge and storage mechanisms, but are also safer for the environment and of lower cost compared to materials in commonly used lithium-ion batteries. Cross-linked Poly(3)-vinyl-N-methylphenothiazine (X-PVMPT) is a p-type OAM which shows high performance and enables fast and reversible energy storage in different battery configurations. The performance of an OAM does not only depend on its molecular or polymer structure, but also on the structure of the composite electrode. The porous nanostructure of an electrode composed of X-PVMPT, a conductive carbon additive and binder is investigated by statistical image analysis, based on 3D image data obtained by focused-ion beam scanning-electron microscopy (FIB-SEM) measurements. Univariate probability distributions of relevant morphological descriptors as well as bivariate distributions of pairs of such descriptors are parametrically modelled, among others, by utilization of copulas in the latter case. These models are then used for quantifying local heterogeneities of X-PVMPT considered in this paper. Furthermore, it is shown that the nanostructure changes when traversing from bottom to top face of the electrode, which influences its performance. While the observed short transportation paths trough the solid phase are beneficial in terms of electrical conductivity, the pathways through the pore phase influencing the effective ionic diffusivity are--in comparison--rather long.

==> SupplementaryMaterial.tex <==
\setcounter{page}{1}
\section*{Supplementary information}


\subsection*{Details of image segmentation}

For image segmentation, i.e., for classifying the voxels as pores or solid, the following features are used: Gaussian smoothing, Laplacian of Gaussian, Gaussian gradient magnitude, difference of Gaussians, structure tensor eigenvalues, and Hessian of Gaussian eigenvalues, each one for $\sigma \in \{0.3,0.7,1.0,1.6,3.5,5.0,10.0\}$. The output of the trained random forests is a probability map, indicating the probability whether a voxel belongs to the pore space or to the solid phase. Each voxel that belongs to the solid phase with probability greater than 0.4 is assigned to solid phase and otherwise to background, leads to a segmentation into the solid phase and its complement. Note that this threshold has been manually determined
based on visual inspection, where we used the open-source software Fiji. 

\subsection*{Univariate probability density functions}


The probability density functions $f:\R\to[0,\infty)$ of the distributions introduced in Section~\ref{sec:uni.den.sin} and used to model the univariate distributions of local morphological descriptors in Section~\ref{sec:univdist} are provided in the following.


\begin{enumerate}

\item Mixture of two Beta distributions $\mathsf{Beta}(\alpha_1, \alpha_2, \beta_1, \beta_2, p_B)$ 
 \begin{equation*}
    f\left(x\right) = p_B\;\frac{\Gamma\left(\alpha_1+\beta_1\right)x^{\alpha_1-1}\left(1-x\right)^{\beta_1-1}}{\Gamma\left(\alpha_1\right)\Gamma\left(\beta_1\right)} +\left(1-p_B\right)\;\frac{\Gamma\left(\alpha_2+\beta_2\right)x^{\alpha_2-1}\left(1-x\right)^{\beta_2-1}}{\Gamma\left(\alpha_2\right)\Gamma\left(\beta_2\right)}, 
\end{equation*} 
for each $x \in [0,1]$, where $\alpha_1, \alpha_2, \beta_1, \beta_2 > 0$ and $0 \leq p_B \leq 1$.

\item
Mixture of two Gaussian distributions $\mathsf{N}(\mu_1, \mu_2, \sigma_1, \sigma_2, p_N)$

\begin{equation*}
    f\left(x\right) = p_N\;\frac{1}{\sigma_1\sqrt{2 \pi}}\exp\left(\frac{\left(x-\mu_1\right)^2}{2\sigma_1^2}\right) + \left(1-p_N\right)\;\frac{1}{\sigma_2\sqrt{2\pi}}\exp\left(\frac{\left(x-\mu_2\right)^2}{2\sigma_2^2}\right)
\end{equation*}
for each $x \in \R$, where $\mu_1, \mu_2 \in \R, \sigma_1, \sigma_2 > 0$ and $0 < p_N < 1.$

\item
Maxwell-Boltzmann distribution $\mathsf{MB}(\mu_{M}, \sigma_{M})$
\begin{equation*}
    f\left(x\right) = \sqrt{\frac{2}{\pi}}\frac{(x-\mu_{M})^2}{\sigma_{M}^2}\exp\left(-\frac{(x-\mu_{M})^2}{2\sigma_{M}^2}\right), 
\end{equation*} 
for each $x>\mu_{M}$, where $\mu_{M} \in \R$ and $\sigma_{M} > 0.$



\item
Shifted Gamma distribution $\Gamma(a_\Gamma, \sigma_\Gamma, \mu_\Gamma)$
\begin{equation*}
     f\left(x\right) = \frac{1}{\Gamma\left(a_\Gamma\right)}\left(\frac{x-\mu_\Gamma}{\sigma_\Gamma}\right)^{a_\Gamma-1}\exp\left(-\frac{x-\mu_\Gamma}{\sigma_\Gamma}\right),
 \end{equation*}
for each $x>\mu_\Gamma,$ where $a_\Gamma, \sigma_\Gamma > 0$ and $\mu_\Gamma \in \R.$

\item
Rayleigh distribution $\mathsf{R}(\mu_R, \sigma_R)$
\begin{equation*}
    f\left(x\right) = \frac{x-\mu_R}{\sigma_R}\exp\left(-\frac{(x-\mu_R)^2}{2\sigma_R^2}\right),
\end{equation*}
for each $x > \mu_R,$ where $\mu_R \in \R$ and $\sigma_R > 0.$

\subsection*{Brief introduction to copulas}


We briefly recall the concept of copulas.  Let $\left(U,V\right)$ be a two-dimeensional random vector taking values in the unit square $[0,1]^2$, where $U$ and $V$ are uniformly distributed on the unit interval $[0,1]$. Then, the joint probability distribution function $C: [0,1]^2 \rightarrow [0,1]$  of $\left(U,V\right)$ is called a two-dimensional copula, where $C(u,v) = P(U \leq u,V \leq v)$ with $P(U\leq u) = u$ and $P(V \leq v)= v$ for any $u,v\in [0,1]$.  
From Sklar's representation formula~\cite{nelsen.2007} we get that for any two-dimensional random vector $(X,Y)$, its  joint probability distribution function $H:\R^2\to[0,1]$ with $H(x,y)=P(X\le x, Y\le y)$  can be written in the form
$$
H(x,y) = C\left(F\left(x\right),G\left(y\right)\right)
$$
for all $x,y \in \mathbb{R}$, where $F:\mathbb{R} \rightarrow [0,1]$ with $F\left(x\right) = P\left(X\leq x\right)$ for each $x \in \R$ and $G:\mathbb{R} \rightarrow [0,1]$ with $G\left(y\right) = P\left(Y\leq y\right)$ for each $y \in \R$ are the univariate distribution functions of $X$ and $Y$, respectively, and $C:[0,1]^2\to[0,1]$ is a certain copula. Moreover, if the functions $F,G$ and $C$ are differentiable, then    the joint probability density $h:\mathbb{R}^2 \rightarrow [0,\infty)$  of $(X,Y)$  can be written as
\begin{equation*}\label{eq:bivariate}
    h(x,y) = f(x)g(y)\left(\frac{\partial^2}{\partial x\partial y}C\right)(F(x),G(y)) 
\end{equation*}
for all $x,y \in \mathbb{R}$, where $f:\mathbb{R} \rightarrow [0,\infty)$ and $g:\mathbb{R} \rightarrow [0,\infty)$ are the univariate probability densities of $X$ and $Y$, respectively. From the joint probability density, we directly obtain the conditional probability density $h_{Y=y}:\mathbb{R} \rightarrow [0, \infty)$ of $X$ given $Y=y$ for each $y \in \R$ fulfilling $g(y) > 0$. It reads as
$$h_{Y=y}(x) = f(x)\left(\frac{\partial^2}{\partial x\partial y}C\right)(F(x),G(y))$$ for each $ x \in \mathbb{R}.$


\end{enumerate}
